The case for a minute-long merger-driven gamma-ray burst from fast-cooling synchrotron emission

For decades, gamma-ray bursts (GRBs) have been broadly divided into `long'- and `short'-duration bursts, lasting more or less than 2s, respectively. However, this dichotomy does not map perfectly to the two progenitor channels that are known to produce GRBs -- the merger of compact objects (merger-GRBs) or the collapse of massive stars (collapsar-GRBs). In particular, the merger-GRBs population may also include bursts with a short, hard $\lesssim$2s spike and subsequent longer, softer extended emission (EE). The recent discovery of a kilonova -- the radioactive glow of heavy elements made in neutron star mergers -- in the 50s-duration GRB 211211A further demonstrates that mergers can drive long, complex GRBs that mimic the collapsar population. Here we present a detailed temporal and spectral analysis of the high-energy emission of GRB 211211A. We demonstrate that the emission has a purely synchrotron origin, with both the peak and cooling frequencies moving through the $\gamma$-ray band down to the X-rays, and that the rapidly-evolving spectrum drives the EE signature at late times. The identification of such spectral evolution in a merger-GRB opens avenues for diagnostics of the progenitor type.

==> affiliation.tex <==
\newcommand{\NU}{\affiliation{Center for Interdisciplinary Exploration and Research in Astrophysics and Department of Physics and Astronomy, \\ Northwestern University, 2145 Sheridan Road, Evanston, IL 60208-3112, USA}}

\newcommand{\Steward}{\affiliation{Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}}

\newcommand{\Leicester}{\affiliation{School of Physics and Astronomy, University of Leicester, University Road, Leicester, LE1 7RH, UK}}

\newcommand{\Radboud}{\affiliation{Department of Astrophysics/IMAPP, Radboud University, 6525 AJ Nijmegen, The Netherlands}}

\newcommand{\Birmingham}{\affiliation{School of Physics and Astronomy,
University of Birmingham,
Birmingham, B15 2TT, UK}}

\newcommand{\BirminghamGW}{\affiliation{Institute for Gravitational Wave Astronomy, University of Birmingham, Birmingham, B15 2TT, UK}}

\newcommand{\CotedeAzur}{\affiliation{Artemis, Universit'e C\^ote d'Azur, Observatoire de la C\^ote d'Azur, CNRS, F-06304 Nice, France}}

\newcommand{\CCA}{\affiliation{Center for Computational Astrophysics, Flatiron Institute, 162 W. 5th Avenue, New York, NY 10011, USA}}

\newcommand{\Columbia}{\affiliation{Department of Physics and Columbia Astrophysics Laboratory, Columbia University, New York, NY 10027, USA}}

\newcommand{\INAFBologna}{\affiliation{INAF - Osservatorio di Astrofisica e Scienza dello Spazio, Via Piero Gobetti 93/3, 40129 Bologna, Italy}}

\newcommand{\INAFRomo}{\affiliation{Osservatorio Astronomico di Roma, via Frascati 33, 00040 Monte Porzio Catone, Italy}}

\newcommand{\MilanoBicocca}{\affiliation{@Maria, please add!}}

\newcommand{\NBIDAWNone}{\affiliation{Cosmic Dawn Center (DAWN), Denmark}}
\newcommand{\NBIDAWNtwo}{\affiliation{Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2200
Copenhagen N, Denmark}}

==> authors.tex <==
\author[0000-0002-9267-6213]{J. C.~Rastinejad}
\NU

\author[0000-0001-7821-9369]{A. J. Levan}
\Radboud

\author[0000-0002-2555-3192]{M. Nicholl}
\Birmingham\BirminghamGW

\author[0000-0002-7374-935X]{W.~Fong}
\NU

\author[0000-0002-5826-0548]{B. P. Gompertz}
\Birmingham\BirminghamGW

\author[0000-0001-5169-4143]{G. P. Lamb}
\Leicester

\author[0000-0002-7517-326X]{D. B. Malesani}
\Radboud\NBIDAWNone\NBIDOWNtwo

\author[0000-0002-2028-9329]{A. E.~Nugent}
\NU

\author[0000-0001-9309-7873]{S. R. Oates}
\Birmingham\BirminghamGW

\author[0000-0003-3274-6336]{N. R. Tanvir}
\Leicester

\author{A. de Ugarte Postigo}
\CotedeAzur

\author[0000-0002-5740-7747]{C. D. Kilpatrick} 
\NU

\author{C. Moore}
\Birmingham\BirminghamGW

\author[0000-0002-4670-7509]{B.~D.~Metzger}
\CCA\Columbia

\author{M. Ravasio}
\Radboud

\author{A. Rossi}
\INAFBologna


\author[0000-0003-3937-0618]{Alicia Rouco Escorial}
\NU

\author{G. Schroeder}
\NU

\author{J. Jencson}
\Steward

\author[0000-0003-4102-380X]{D.~J. Sand}
\Steward

\author[0000-0001-5510-2424]{N. Smith}
\Steward

\author{alphabetized, opt-in}

\author[0000-0001-8340-3486]{K. Paterson}
\affil{Max-Planck-Institut f\"ur Astronomie (MPIA), Königstuhl 17, 69117 Heidelberg, Germany}

% Program Co-I's not at core meetings: 
% Gemini: Edo Berger, Brad Cenko, Ryan Chornock, Nino Cucchiara, Charlie Kilpatrick, Bethany Cobb Kung, Kerry Paterson, Daniel Perley, Alicia Rouco Escorial

% MMT (NU program): Peter Blanchard, Kate Alexander, Genevieve Schroeder, Anya Nugent

% MMT (Aztec program): Dave Sand, Jacob Jencson, Nathan Smith

% Keck: Adam Miller

% VLA: Tanmoy Laskar

% CAHA + GTC: José Feliciano Agüí Fernández, Christina Thöne, David Alexander Kann and Antonio de Ugarte Postigo
% A. de Ugarte Postigo
% 	Artemis, Universit'e C\^ote d'Azur, Observatoire de la C\^ote d'Azur, CNRS, F-06304 Nice, France
% C. C. Th\“one
% 	Astronomical Institute of the Czech Academy of Sciences (ASU-CAS), Fri\v cova 298, 251 65 Ond\v rejov, Czech Republic
% D. A. Kann
% J. F. Ag\“u\’i Fern\’andez
% 	Instituto de Astrof\’isica de Andaluc\’ia, Glorieta de la Astronom\’ia,E-18008, Granada, Spain

% NOT: Johan Fynbo <jfynbo@nbi.ku.dk>, L. Izzo <luca.izzo@nbi.ku.dk>

% LBT: Andrea Rossi, Ester Marini
% Andrea Rossi, andrea.rossi@inaf.it
% INAF - Osservatorio di Astrofisica e Scienza dello Spazio, Via Piero Gobetti 93/3, 40129 Bologna, Italy
% Ester Marini, ester.marini@inaf.it,
% INAF - Osservatorio Astronomico di Roma, via Frascati 33, 00040 Monte Porzio Catone, Italy

